The Curse of Diversity in Ensemble-Based Exploration

We uncover a surprising phenomenon in deep reinforcement learning: training a diverse ensemble of data-sharing agents -- a well-established exploration strategy -- can significantly impair the performance of the individual ensemble members when compared to standard single-agent training. Through careful analysis, we attribute the degradation in performance to the low proportion of self-generated data in the shared training data for each ensemble member, as well as the inefficiency of the individual ensemble members to learn from such highly off-policy data. We thus name this phenomenon the curse of diversity. We find that several intuitive solutions -- such as a larger replay buffer or a smaller ensemble size -- either fail to consistently mitigate the performance loss or undermine the advantages of ensembling. Finally, we demonstrate the potential of representation learning to counteract the curse of diversity with a novel method named Cross-Ensemble Representation Learning (CERL) in both discrete and continuous control domains. Our work offers valuable insights into an unexpected pitfall in ensemble-based exploration and raises important caveats for future applications of similar approaches.

==> algorithms/bootdqn_individual.tex <==

\begin{algorithmic}
    \Require total interaction steps $M$, $N$ value functions $\{Q_i(s, a;\theta)\}_{i=1}^N$
    % \REPEAT
    \State $t\gets \mathrm{True}$ 
    \Comment{Terminal state indicator/whether to start a new episode}
    \For{$m \gets 1$ \textbf{to} $M$}
        \If{$t = \mathrm{True}$}
            \Comment{New episode}
            \State $s_m\gets \mathrm{reset}(\mathrm{env})$
            \State $k \sim \mathrm{Uniform}(\{1,\ldots, N\})$
            \Comment{Randomly sample a member for acting}
        \Else
            \State $s_m \gets s_{m-1}'$
        \EndIf
        \State $a_m\gets \arg\max_a Q_k(s_m, a;\theta)$
        \State $a_m\sim \operatorname{\epsilon-\mathrm{greedy}}(a_m)$
        \Comment{Epsilon greedy policy during evaluation}
        \State     $s_m'$, $r_m$, $t_m$ $\gets \mathrm{step}(\mathrm{env}, a_m)$
    \EndFor
    % \UNTIL{$noChange$ is $true$}
\end{algorithmic}

==> algorithms/bootdqn_voting.tex <==

\begin{algorithmic}
    \Require total interaction steps $M$, $N$ value functions $\{Q_i(s, a;\theta)\}_{i=1}^N$
    % \REPEAT
    \State $t\gets \mathrm{True}$ 
    \Comment{Terminal state indicator/whether to start a new episode}
    \For{$m \gets 1$ \textbf{to} $M$}
        \If{$t = \mathrm{True}$}
            \Comment{New episode}
            \State $s_m\gets \mathrm{reset}(\mathrm{env})$
        \Else
            \State $s_m \gets s_{m-1}'$
        \EndIf
        \For{$i \in \{1, \ldots, N\}$}
            \State $\va_m^{(i)} = \operatorname{one\_hot}( \arg\max_a Q_i(s_m, a;\theta))$
            \Comment{One-hot encoding of the actions}
        \EndFor
        
        
        \State $a_m\gets \arg\max_a [\sum_{i=1}^N \va_m^{(i)}]_a$
        \Comment{Get the action with the most votes}
        \State $a_m\sim \operatorname{\epsilon-\mathrm{greedy}}(a_m)$ 
        \Comment{Epsilon greedy policy during evaluation}
        \State     $s_m'$, $r_m$, $t_m$ $\gets \mathrm{step}(\mathrm{env}, a_m)$
    \EndFor
    % \UNTIL{$noChange$ is $true$}
\end{algorithmic}

==> tables/games.tex <==
\begin{tabular}{llllll}
\toprule 
 \textsc{Alien}      & \textsc{Breakout}        & \textsc{Kung Fu Master} & \textsc{Seaquest}       \\
 \textsc{Amidar}     & \textsc{Chopper Command} & \textsc{Ms Pacman}      & \textsc{Space Invaders} \\
 \textsc{Assault}    & \textsc{Demon Attack}    & \textsc{Name This Game} & \textsc{Star Gunner}    \\
 \textsc{Asterix}    & \textsc{Gravitar}        & \textsc{Qbert}          & \textsc{Time Pilot}     \\
 \textsc{Atlantis}   & \textsc{Kangaroo}        & \textsc{Riverraid}      & \textsc{Wizard Of Wor}  \\
 \textsc{Beam Rider} & \textsc{Krull}           & \textsc{Road Runner}    & \textsc{Yars Revenge}   \\

\bottomrule
\end{tabular}

